REPQC: Reverse Engineering and Backdooring Hardware Accelerators for Post-quantum Cryptography

Significant research efforts have been dedicated to designing cryptographic algorithms that are quantum-resistant. The motivation is clear: robust quantum computers, once available, will render current cryptographic standards vulnerable. Thus, we need new Post-Quantum Cryptography (PQC) algorithms, and, due to the inherent complexity of such algorithms, there is also a demand to accelerate them in hardware. In this paper, we show that PQC hardware accelerators can be backdoored by two different adversaries located in the chip supply chain. We propose REPQC, a sophisticated reverse engineering algorithm that can be employed to confidently identify hashing operations (i.e., Keccak) within the PQC accelerator - the location of which serves as an anchor for finding secret information to be leaked. Armed with REPQC, an adversary proceeds to insert malicious logic in the form of a stealthy Hardware Trojan Horse (HTH). Using Dilithium as a study case, our results demonstrate that HTHs that increase the accelerator's layout density by as little as 0.1\% can be inserted without any impact on the performance of the circuit and with a marginal increase in power consumption. An essential aspect is that the entire reverse engineering in REPQC is automated, and so is the HTH insertion that follows it, empowering adversaries to explore multiple HTH designs and identify the most suitable one.

==> preamble.tex <==
\usepackage{cite}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{tikz}
\usepackage{tikzsymbols}
\usetikzlibrary{positioning, shapes.geometric, arrows,patterns,decorations.markings,pgfplots.groupplots}
\usepackage{pgfplots,pgfplotstable} 
    \usepgfplotslibrary{statistics}
    
    
\usepackage{algorithm}
\usepackage{algpseudocode} 
\usepackage{amsthm}

\usepackage{tablefootnote}

\usepackage{multirow}
\usepackage{makecell}

\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{color}
\usepackage[]{hyperref}
\usepackage[]{caption}
\usepackage{subcaption}
\usepackage{pifont}% http://ctan.org/pkg/pifont
%\newcommand{\cmark}{\ding{51}}%
%\newcommand{\xmark}{\ding{55}}%

\pgfmathdeclarefunction{gauss}{2}{%
  \pgfmathparse{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))}%
}

\renewcommand\theadalign{bc}
\renewcommand\theadfont{\bfseries}
%\renewcommand\theadgape{\Gape[4pt]}
%\renewcommand\cellgape{\Gape[4pt]}

\usepackage{circuitikz}
\usetikzlibrary{spy, calc}

\usepackage{adjustbox}

\definecolor{mycolor1}{RGB}{251,180,174}
\definecolor{mycolor2}{RGB}{179,205,227}
\definecolor{mycolor3}{RGB}{204,235,197}
\definecolor{mycolor4}{RGB}{222,203,228}
\definecolor{mycolor5}{RGB}{254,217,166}
\definecolor{mycolor6}{RGB}{255,255,204}
\definecolor{wildstrawberry}{rgb}{1.0, 0.26, 0.64}

%\overfullrule=1mm %todo this helps to visualize overfull boxes. can be removed for final submission

\pgfplotsset{compat=1.18} 
